Developing Theoretical Foundations for Runtime Enforcement

The ubiquitous reliance on software systems increases the need for ensuring that systems behave correctly and are well protected against security risks. Runtime enforcement is a dynamic analysis technique that utilizes software monitors to check the runtime behaviour of a software system with respect to a correctness specification. Whenever the runtime behaviour of the monitored system is about to deviate from the specification (either due to a programming bug or a security hijack attack), the monitors apply enforcement techniques to prevent this deviation. Current Runtime Enforcement techniques require that the correctness specification defines the behaviour of the enforcement monitor itself. This burdens the specifier with not only having to define property that needs to be enforced, but also with having to specify how this should be enforced at runtime; we thus relieve the specifier from this burden by resorting to a highly expressive logic. Using a logic we allow the specifier to define the correctness specification as a logic formula from which we can automatically synthesise the appropriate enforcement monitor. Highly expressive logics can, however, permit for defining a wide variety of formulae, some of which cannot actually be enforced correctly at runtime. We thus study the enforceability of Hennessy Milner Logic with Recursion for which we identify a subset that allows for defining enforceable formulae. This allows us to define a synthesis function that translates enforceable formulae into enforcement monitors. As our monitors are meant to ensure the correct behaviour of the monitored system, it is imperative that they work correctly themselves. We thus study formal definitions that allow us to ensure that our enforcement monitors behave correctly.

==> sections/correctness.tex <==
\begin{itemize}
	\item We show that our enforcement monitors are correct by following in the footsteps of earlier research \cite{Ligatti2005,Bielova2011,Falcone2009EM} and proving \emph{Soundness} and \emph{Transparency}.
	\item We also prove that well-formed \shml properties are synthesised into \emph{deterministic enforcement monitors}.
\end{itemize}

\input{sections/determinism-proof-V2.tex}
	
\input{sections/soundness-proof-V3.tex}
	
\input{sections/transparency-proof-V3.tex}	
	

==> sections/rel-enf-mon.tex <==
Although it is generally assumed that logic formulae that are enforceable via enforcer are also monitorable via detection monitors, to our knowledge, no one has yet established a formal relationship between the monitorability and enforceability of formulae. We conjuncture that \uhml formulae that are \emph{strongly enforceable} via suppression enforcers are also monitorable \wrt \Cref{def:monitrability}. In this section we therefore define a formal relation between the definition of monitorability of \uhml formulae presented in \cite{Francalanza2015Mon}, and our definition of strong enforceability introduced in \Cref{sec:enforceability}.

To develop such a relation we start by differentiating between \emph{negative and positive detection monitors} (\nmondef{\mV}{\hV} and \pmondef{\mV}{\hV} \resp), \ie monitors that issue violations (\resp satisfaction) verdicts only, as defined in \Cref{def:neg-pos-mon}. 

\begin{definition}[Positive and Negative Monitoring] \label{def:neg-pos-mon} 
	\begin{addmargin}[1cm]{0cm}
		\begin{align*}
			\pmondef{\mV}{\hV} & \defeq \; 
				\begin{xbrace}{l}
%					\forall \pV\cdot \pV\!\in\!\syn{\hV}\;\imp\;\monacc{\pV}{\mV}\\
%					\monacc{\pV}{\mV}\;\imp\;\forall \pV\cdot \pV\!\in\!\syn{\hV}	
					\forall \pV\cdot \pV\vSat\hV\;\imp\;\monacc{\pV}{\mV}\\
					\monacc{\pV}{\mV}\;\imp\;\forall \pV\cdot \pV\vSat\hV	
				\end{xbrace} && \hfill \text{(positive)} & \\[3mm]
			\nmondef{\mV}{\hV} & \defeq \; 
				\begin{xbrace}{l}
%					\forall \pV\cdot \pV\!\notin\!\syn{\hV}\;\imp\;\monrej{\pV}{\mV}\\
%					\monrej{\pV}{\mV}\;\imp\;\forall \pV\cdot \pV\!\notin\!\syn{\hV}
					\forall \pV\cdot \pV\nvSat\hV\;\imp\;\monrej{\pV}{\mV}\\
					\monrej{\pV}{\mV}\;\imp\;\forall \pV\cdot \pV\nvSat\hV	
				\end{xbrace} && \hfill \text{(negative)}& 
		\end{align*} \\[-15mm]\bqed
	\end{addmargin}
\end{definition} 
Using these definitions we create an alternative definition for monitorability (in \Cref{def:alt-mon}) which states that a property \hV is monitorable either if there exists a monitor that can find a \emph{violation} for the given property (\ie \nmondef{\mV}{\hV}) \emph{or} else if there exists a monitor that can find a \emph{satisfaction} (\ie \pmondef{\mV}{\hV}). 
\begin{definition}[Monitorability (Alternative)]
	\label{def:alt-mon}  % Property
	$\\$Formula \hV is \emph{monitorable} iff there exists a monitor $\mV$  such that $\amondef{\mV}{\hV}$, where $\amondef{\mV}{\hV} \defeq \pmondef{\mV}{\hV}\text{ or }\nmondef{\mV}{\hV}.$ \bqed
\end{definition}
We then prove that \Cref{def:alt-mon} corresponds to \Cref{def:mon-form-corr} by proving \Cref{thm:amon-mon} (see \Cref{sec:app:rel-mon-amon-proof} for full proof).
\begin{theorem}[Correspondence of Definitions] \label{thm:amon-mon}
	$\\$\indent$\forall\hV\in\uhml,\mV\in\Mon\cdot\,\mondef{\mV}{\hV}\textsl{  iff  }\amondef{\mV}{\hV}$ \bqed
\end{theorem}

This allows us to show that properties that are \emph{strongly enforceable} via suppression monitors are also \emph{negatively monitorable} as defined in \Cref{def:enf-amon}. Hence, this definition establishes a relationship between monitorable and enforceable \uhml properties, by stating that for every suppression enforcer \eV that strongly enforces a formula \hV, we can find a detection monitor \mV that can detect violations for \hV.

\begin{definition}[Enforceability-Monitorability Relation] \label{def:enf-amon}
	$\\$\indent$\enfmonrel{\eV}{\mV}\,\defeq\,\forall\hV\in\uhml,\eV\in\Enf\cdot\,\enfdef{\eV}{\hV}\imp\exists\mV\cdot\nmondef{\mV}{\hV}$ \bqed
\end{definition}

To prove the relation defined in \Cref{def:enf-amon} actually exists within our setting, we prove that: any \uhml formula \hV that can be derived into an enforcer \eV by the synthesis function given in \Cref{fig:enf-synthesis} and be strongly enforced by it, can also be converted into a detection monitor \mV using the synthesis in \Cref{fig:mon-synthesis} \cite{Francalanza2015Mon} and be negatively monitorable by the synthesised monitor. To ensure this we prove that \Cref{thm:syn-enf-mon-rel} holds; see \Cref{sec:app:rel-mon-enf-proof} for the full proof.

\begin{theorem}[Relating Synthesised Enforcers to Monitors]\label{thm:syn-enf-mon-rel}
%	\begin{center}
	$\\$\indent$\enfmonrel{\g{\hV}}{\gRV{\hV}}$
%	\end{center} 
\vspace{-6mm}\bqed
\end{theorem}
 \vspace{-8mm}

==> sections/shml-normalization-full-example.tex <==
\subsection{A complete Normalization example}
In this section we provide a complete example on how a simple \shml formula $\hV$ is converted into an equivalent \shmlwf formula $\hV^{\textsf{wf}}$. Note that the end result of each derivation is obtained in a compositional manner, \ie the initial equation is subdivided into smaller parts (subequations) and analysed accordingly. The results of these sub-equations are then used to obtain the end result.\\

\noindent Consider the following \shml formula:
$$ \hV = \hmax{\hVarX_0}{\hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}\hVarX_0\hand\hnec{\recv{i}{x_3}}\hgnec{\recv{x_4}{5}}{x\!\notin\!\Set{i,j}}\hfls} $$

\begin{derivation}[Step 1 - Convert to Standard Form using Construction~\ref{sec-form-to-sfform}]
$\\[-8mm]$	 \normalfont
\newcommand{\formA}{\hmax{\hVarX_0}{\formB}}
\newcommand{\formB}{\formBa\hand\formBb}
\newcommand{\formBa}{\hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}\hVarX_0}
\newcommand{\formBb}{\hnec{\recv{i}{x_3}}\hgnec{\recv{x_4}{5}}{x_4\!\notin\!\set{i,j}}\hfls}

\newcommand{\formAP}{\hmax{\hVarX_0}{\formBP}}
\newcommand{\formBP}{\formBaP\hand\formBbP}
\newcommand{\formBaP}{\hnec{\recv{x_1'}{5}}\hgnec{\recv{j}{x_2'}}{x_2'\!>\!3}\hVarX_0}
\newcommand{\formBbP}{\hnec{\recv{i}{x_3'}}\hgnec{\recv{x_4'}{5}}{x_4'\!\notin\!\Set{i,j}}\hfls}
\begin{flushleft}
Since $\hV=\hmax{\hVarX}{\hV'}$ we know
$$\gensf{\hmax{\hVarX}{\hV'}} = \hVV\Sub{\hmax{\hVarX}{(\hVV\hand\hAND{j\in\f{\hVV}\setminus\set{j}=\emptyset\hspace{-13mm}}\hVarX_j)} }{\hVarX} \qquad\qquad \text{  where } \gensf{\hV'}=\hVV\hand\hAND{i\in\f{\hV'}\hspace{-5mm}}\hVarX_i$$ 
Since $\hV'=\formB$ we know
$$\gensf{\formB} = (\hVV_1\hand\hVV_2)\hand\!\!\!\hAND{j\in\f{\hVV_1}\cup\f{\hVV_2}=\emptyset\hspace{-18mm}}\hVarX_j$$
where $\gensf{\formBa}=\formBa\hand\hAND{j\in\emptyset}\hVarX_j$ and\\ \qquad\qquad$\gensf{\formBb}=\formBb\hand\hAND{j\in\emptyset}\hVarX_j$. \\[2mm]

Hence, the resultant formula is the following:
$$\begin{array}{rcl}
	\gensf{\hV} &=& (\formB\hand\!\!\hAND{j\in\emptyset}\!\hVarX_j)\sub{\formA}{\hVarX_0} \\
	&=& \hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}(\formAP)\hand\formBb
\end{array}$$
\end{flushleft}
\end{derivation}
\vspace{5mm}


\begin{derivation}[Step 2 - Convert to a System of Equations in Standard Form using Construction~\ref{sec-sfform-to-sfsys}]
	$\\[-10mm]$	 \normalfont
	\newcommand{\formA}{\hmax{\hVarX_0}{\formB}}
	\newcommand{\formB}{\formBa\hand\formBb}
	\newcommand{\formBa}{\hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}\hVarX_0}
	
	\newcommand{\formBbb}{\hfls}
	\newcommand{\formBba}{\hgnec{\recv{x_4}{5}}{x\!\notin\!\Set{i,j}}\formBbb}
	\newcommand{\formBb}{\hnec{\recv{i}{x_3}}\formBba}
	\newcommand{\formAP}{\hmax{\hVarX_0}{(\formBP)}}
	\newcommand{\formBP}{\formBaP\hand\formBbP}
	
	\newcommand{\formBaPa}{\hgnec{\recv{j}{x_2'}}{x_2'\!>\!3}\hVarX_0}
	\newcommand{\formBaP}{\hnec{\recv{x_1'}{5}}\formBaPa}
	
	\newcommand{\formBbPa}{\hgnec{\recv{x_4'}{5}}{x_4'\!\notin\!\Set{i,j}}\hfls}
	\newcommand{\formBbP}{\hnec{\recv{i}{x_3'}}\formBbPa}	
	
	\newcommand{\formAAa}{\hgnec{\recv{j}{x_2}}{x_2\!>\!3}(\formAP)}
	\newcommand{\formAA}{\hnec{\recv{x_1}{5}}\formAAa}
	\newcommand{\formula}{\formAA\hand\formBb}
	
	\newcommand{\XThirteen}{\hVarX_{13} = \hnec{\recv{x_1}{5}}\hVarX_{11} \hand \hnec{\recv{i}{x_3}}\hVarX_2}
	\newcommand{\XTwelve}{\hVarX_{12} = \hnec{\recv{x_1}{5}}\hVarX_{11}}
	\newcommand{\XEleven}{\hVarX_{11} = \hgnec{\recv{j}{x_2}}{x_2>3}\hVarX_0}
	\newcommand{\XTen}{\hVarX_{10} = \hnec{\recv{x_1'}{5}}\hVarX_5 \hand \hnec{\recv{i}{x_3'}}\hVarX_8}
	\newcommand{\XNine}{\hVarX_9 = \hnec{\recv{i}{x_3'}}\hVarX_8}
	\newcommand{\XEight}{\hVarX_8 = \hgnec{\recv{x_4'}{5}}{x_4'\!\notin\!\Set{i,j}}\hVarX_7}
	\newcommand{\XSeven}{\hVarX_7 = \hfls}
	\newcommand{\XSix}{\hVarX_6 = \hnec{\recv{x_1'}{5}}\hVarX_5}
	\newcommand{\XFive}{\hVarX_5 = \hgnec{\recv{j}{x_2'}}{x_2'\!>\!3}\hVarX_4}
	\newcommand{\XFour}{\hVarX_4 = \hVarX_0}
	\newcommand{\XThree}{\hVarX_3 = \hnec{\recv{i}{x_3}}\hVarX_2}
	\newcommand{\XTwo}{\hVarX_2 = \hgnec{\recv{x_4}{5}}{x_4\!\notin\!\Set{i,j}}\hVarX_1}
	\newcommand{\XOne}{\hVarX_1 = \hfls}	
	\newcommand{\XZero}{\hVarX_0 = \hnec{\recv{x_1'}{5}}\hVarX_5 \hand \hnec{\recv{i}{x_3'}}\hVarX_8}
	
	\begin{flushleft}
		Consider the standard form \shml formula obtained in the previous step.
		$$\hV_{\textsf{sf}} = \formula$$
		
		Since $\hV_{\textsf{sf}}=\hV_1\hand\hV_2$ we know  
		$$\gensys{\hV_1\hand\hV_2} =\;\; \syseq{\Set{\hVarX_{13}=\eq_2(\hVarX_{12})\hand\eq_1(\hVarX_{3})}\cup \eq_1\cup \eq_2}{\hVarX_{13}}{\sysrecsetE}$$
		where $\gensys{\hV_1}=\syseq{\eq_1}{\hVarX_{3}}{\sysrecsetE}$ and $\gensys{\hV_2}=\syseq{\eq_2}{\hVarX_{12}}{\sysrecsetE}$.\\[5mm]
		
		Since we have $\gensys{\hV_1}$ (LHS) and $\gensys{\hV_2}$ (RHS), we must evaluate them separately. 
			
			\textbf{\underline{RHS:}}\\[2mm]
			\begin{context}
				Since  $\hV_2=\formBb$ we know
				$$\gensys{\formBb} = \syseq{\eq_1 = \Set{\XOne,\XTwo,\XThree}}{\hVarX_{3}}{\sysrecsetE}$$
			\end{context}
		
			\textbf{\underline{LHS:}}\\[2mm]
			\begin{context}
				Since  $\hV_1=\hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}\hV_1'$ we know
				$$\gensys{\hnec{\recv{x_1}{5}}\hgnec{\recv{j}{x_2}}{x_2\!>\!3}\hV_1'}=\syseq{Eq_1'\cup\Set{\XEleven,\XTwelve}}{\hVarX_{12}}{\sysrecsetE}$$
				where $\gensys{\hV_1'}=\syseq{\eq_1'}{\hVarX_{0}}{\sysrecsetE}$
				\\[3mm]
			
				Since  $\hV_1'=\hmax{\hVarX_0}{\hV_1''}$ we know
				$$\gensys{\hmax{\hVarX_0}{\hV_1''}} = \syseq{\Set{\hVarX_{0}=\eq_1''(\hVarX_{10})}\cup\eq_1'' }{\hVarX_{0}}{\sysrecsetE}$$
				where $\gensys{\hV_1''}=\syseq{\eq_1''}{\hVarX_{0}}{\sysrecsetE}$
				\\[3mm]
				
				Since  $\hV_1''=\hV_2\hand\hV_3$ we know
				$$\gensys{\hV_3\hand\hV_4} = \syseq{\Set{\hVarX_{10}=\eq_3(\hVarX_{6})\hand\eq_4(\hVarX_{9})}\cup\eq_3\cup\eq_4 }{\hVarX_{10}}{\Set{\hVarX_{0}}}$$
				where $\gensys{\hV_3}=\syseq{\eq_3}{\hVarX_{6}}{\Set{\hVarX_{0}}}$ and $\gensys{\hV_4}=\syseq{\eq_4}{\hVarX_{9}}{\sysrecsetE}$
				\\[3mm]
				
				Since we have $\gensys{\hV_3}$ (LHS) and $\gensys{\hV_4}$ (RHS), we must evaluate these cases separately. 
								
				\textbf{\underline{LHS:}}\\[2mm]
				\begin{context}
					Since $\hV_3=\formBaP$ we know
					$$\gensf{\formBaP} = \syseq{\Set{\XFour,\XFive,\XSix}}{\hVarX_{6}}{\Set{\hVarX_{0}}}$$
				\end{context}
												
				\textbf{\underline{RHS:}}\\[2mm]
				\begin{context}
					Since $\hV_4=\formBbP$ we know
					$$\gensf{\formBbP} = \syseq{\Set{\XSeven,\XEight,\XNine}}{\hVarX_{9}}{\sysrecsetE}$$
				\end{context}
		\end{context}
	\end{flushleft}\vspace{2mm}
	
\noindent $\therefore$ The Result is $\gensys{\hV_{\textsf{sf}}} \; =\; \syseq{Eq}{X_{13}}{\sysrecsetE}$ where
$$Eq = \begin{mlbrack}
	\XThirteen,&\strike[red]{\XTwelve},\\\XEleven,&\strike[red]{\XTen},\\\strike[red]{\XNine},&\XEight,\\\XSeven,&\strike[red]{\XSix},\\\XFive,&\XFour,\\\strike[red]{\XThree},&\XTwo,\\\XOne, &\XZero
\end{mlbrack}$$

\begin{remark}
	Some equations are crossed out since they are \emph{not reachable} from the initial logical variable $\hVarX_{13}$. These will therefore be ignored in subsequent constructions. 
\end{remark}
\end{derivation}

\begin{derivation}[Step 3 - Convert to a Fully-Open System of Equations using Construction~\ref{sec-fully-open-cons}]
$\\[-8mm]$
\normalfont	
	\newcommand{\XThirteen}{\hVarX_{13} = \hgnec{\recv{x_1}{\pmb{x_5}}}{\pmb{x_5\!=\!5}}\hVarX_{11} \hand \hgnec{\recv{\pmb{x_6}}{x_3}}{\pmb{x_6=i}}\hVarX_2}
	\newcommand{\XEleven}{\hVarX_{11} = \hgnec{\recv{\pmb{x_7}}{x_2}}{(x_2>3\land\pmb{x_7=j})}\hVarX_0}
	\newcommand{\XEight}{\hVarX_8 = \hgnec{\recv{x_4'}{\pmb{x_8'}}}{(x_4'\!\notin\!\Set{i,j}\land \pmb{x_8'=5})}\hVarX_7}
	\newcommand{\XSeven}{\hVarX_7 = \hfls}
	\newcommand{\XFive}{\hVarX_5 = \hgnec{\recv{\pmb{x_7'}}{x_2'}}{(x_2'>3\land\pmb{x_7'=j})}\hVarX_4}
	\newcommand{\XFour}{\hVarX_4 = \hVarX_0}
	\newcommand{\XTwo}{\hVarX_2 = \hgnec{\recv{x_4}{\pmb{x_8}}}{(x_4\!\notin\!\Set{i,j} \land \pmb{x_8=5})}\hVarX_1}
	\newcommand{\XOne}{\hVarX_1 = \hfls}	
	\newcommand{\XZero}{\hVarX_0 = \hgnec{\recv{x_1'}{\pmb{x_5'}}}{\pmb{x_5'=5}}\hVarX_5 \hand \hgnec{\recv{\pmb{x_6'}}{x_3'}}{\pmb{x_6'=i}}\hVarX_8}

\noindent Consider the system of equations obtained in the previous step. By applying the equation reconstruction we obtain
	$$\eqOpen = \begin{mlbrack}
	\XThirteen,&\XEleven,\\\XEight,&\XSeven,\\\XFive,&\XFour,\\\XTwo,&\XOne,\\\XZero
	\end{mlbrack}$$
	Notice how the concrete values in the patterns have been replaced by a \emph{fresh variable} that was then guarded by an equality which states that the value bound to the replacing variable should be equal to the replaced value. For instance the necessity $\hnec{\recv{x_1}{5}}$ defined in equation $\hVarX_{13}$ was reconstructed into $\hgnec{\recv{x_1}{\pmb{x_5}}}{\pmb{x_5\!=\!5}}$, where $x_5$ is a guarded fresh variable. \\
	
	\noindent $\therefore$ The Result is $\genopen{\syseq{Eq}{X_{13}}{\sysrecsetE}} \; =\; \syseq{\eqOpen}{X_{13}}{\sysrecsetE}$	
\end{derivation}

\begin{derivation}[Step 4 - Convert to a Generic System of Equations using Construction~\ref{sec-alpha-equiv-cons}]
	$\\$	 \normalfont
	\noindent Consider the system of equations obtained in the previous step. By applying the Construction~\ref{sec-alpha-equiv-cons} we obtain
	\newcommand{\XThirteen}{\hVarX_{13} = \hgnec{\recv{y_1}{y_2}}{y_2\!=\!5}\hVarX_{11} \hand \hgnec{\recv{y_1}{y_2}}{y_1=i}\hVarX_2}
	\newcommand{\XEleven}{\hVarX_{11} = \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)}\hVarX_0}
	\newcommand{\XEight}{\hVarX_8 = \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)}\hVarX_7}
	\newcommand{\XSeven}{\hVarX_7 = \hfls}
	\newcommand{\XFive}{\hVarX_5 = \hgnec{\recv{y_7}{y_8}}{(y_8>3\land y_7=j)}\hVarX_4}
	\newcommand{\XFour}{\hVarX_4 = \hVarX_0}
	\newcommand{\XTwo}{\hVarX_2 = \hgnec{\recv{y_3}{y_4}}{(y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_1}
	\newcommand{\XOne}{\hVarX_1 = \hfls}	
	\newcommand{\XZero}{\hVarX_0 = \hgnec{\recv{y_5}{y_6}}{y_6=5}\hVarX_5 \hand \hgnec{\recv{y_5}{y_6}}{y_5=i}\hVarX_8}
		
	$$\genalpha{\syseq{\eqOpen}{\hVarX_{13}}{\sysrecsetE}} \;\; = \;\; \syseq{\genalphaEq{\eqOpen}{\Set{13}}{\emptyset}}{\hVarX_{13}}{\sysrecsetE} \qquad \text{    where }$$   
	
	$\\\genalphaEq{\eqOpen}{\Set{13}}{\emptyset}=\Set{\XThirteen}\cup\genalphaEq{\eqOpen^1}{Q_1}{\s}\\$	
	where $\eqOpen^1=\eqOpen\setminus\Set{\hVarX_{13}=F_{13}}$ and $\s_1=[\subE{y_1}{x_1},\subE{y_2}{x_5},\subE{y_1}{x_6},\subE{y_2}{x_3}]$ and $Q_1=\bigunion{i\in\set{13}\hspace{-5mm}}\after{i}\,=\,\Set{11,2}$\\
	
	$\\\genalphaEq{\eqOpen^1}{\Set{11,2}}{\s_1}=\Set{\XEleven}\cup\Set{\XTwo}\cup\genalphaEq{\eqOpen^2}{Q_2}{\s_2}\\$	
	where $\eqOpen^2=\eqOpen^1\setminus\Set{\hVarX_{11}=F_{11},\hVarX_{2}=F_{2}}$ and $\s_2=\s_1\cup[\subE{y_3}{x_7},\subE{y_4}{x_2},\subE{y_3}{x_4},\subE{y_4}{x_8}]$ and $Q_2=\bigunion{i\in\set{11,2}\hspace{-5mm}}\after{i}\,=\,\Set{0,1}$\\
	
	$\\\genalphaEq{\eqOpen^2}{\Set{0,1}}{\s_2}=\Set{\XOne}\cup\Set{\XZero}\cup\genalphaEq{\eqOpen^3}{Q_3}{\s_3}\\$	
	where $\eqOpen^3=\eqOpen^2\setminus\Set{\hVarX_{0}=F_{0},\hVarX_{1}=F_{1}}$ and $\s_3=\s_2\cup[\subE{y_5}{x_2'},\subE{y_6}{x_5'},\subE{y_5}{x_6'},\subE{y_6}{x_3'}]$ and  $Q_3=\bigunion{i\in\set{0,1}\hspace{-5mm}}\after{i}\,=\,\Set{5,8}$\\
	
	$\\\genalphaEq{\eqOpen^3}{\Set{5,8}}{\s_3}=\Set{\XFive}\cup\Set{\XEight}\cup\genalphaEq{\eqOpen^4}{Q_4}{\s_4}\\$
	where $\eqOpen^4=\eqOpen^3\setminus\Set{\hVarX_{5}=F_{5},\hVarX_{8}=F_{8}}$ and $\s_4=\s_3\cup[\subE{y_7}{x_4'},\subE{y_8}{x_8'},\subE{y_7}{x_7'},\subE{y_8}{x_2'}]$ and  $Q_4=\bigunion{i\in\set{5,8}\hspace{-5mm}}\after{i}\,=\,\Set{4,7}$ \\
	
	$\\\genalphaEq{\eqOpen^4}{\Set{4,7}}{\s_4}=\Set{\XFour}\cup\Set{\XSeven}\cup\genalphaEq{\eqOpen^5}{Q_5}{\s_5}\\$
	where $\eqOpen^5=\eqOpen^4\setminus\Set{\hVarX_{4}=F_{4},\hVarX_{7}=F_{7}}=\emptyset$ and $\s_5=\s_4$  and  $Q_5=\bigunion{i\in\set{4,7}\hspace{-5mm}}\after{i}\,=\,\emptyset$ \\
	
	$\\\genalphaEq{\eqE}{\emptyset}{\s_5}=\eqE$	
		
	\noindent $\\[2mm]\therefore$ The Result is $\genalpha{\syseq{\eqOpen}{X_{13}}{\sysrecsetE}} \; =\; \syseq{Eq^\alpha}{X_{13}}{\sysrecsetE}$	 where 	
	$$Eq^\alpha = \begin{mlbrack}
	\XThirteen,&\XEleven,\\\XEight,&\XSeven,\\\XFive,&\XFour,\\\XTwo,&\XOne,\\\XZero
	\end{mlbrack}$$
\end{derivation}\vspace{5mm}

\begin{derivation}[Step 5 - Convert to a Distinctive System of Equations using Construction~\ref{sec-truth-combos-cons}]
	
	$\\[-5mm]$	 \normalfont
	\newcommand{\XThirteen}{\hVarX_{13} = \begin{mlbrace}
			\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_{11} \hand \hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!\neq\!i)}\hVarX_{11} \hand \\ \hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_2 \hand \hgnec{\recv{y_1}{y_2}}{(y_2\!\neq\!5\land y_1\!=\!i)}\hVarX_2
		\end{mlbrace}}
	\newcommand{\XEleven}{\hVarX_{11} =  \begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_0 \hand \\\hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land \lnot(y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_0  \end{mlbrace}}
	\newcommand{\XTwo}{\hVarX_2 =  \begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_1\hand\\ \hgnec{\recv{y_3}{y_4}}{\lnot(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_1 \end{mlbrace}}	
	\newcommand{\XEight}{\hVarX_8 =   \begin{mlbrace} \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_7 \hand \\\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land\lnot(y_8>3\land y_7=j)}\hVarX_7\end{mlbrace}}	
	\newcommand{\XSeven}{\hVarX_7 = \hfls}
	\newcommand{\XFive}{\hVarX_5 = \begin{mlbrace}	\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_4 \\\hand \hgnec{\recv{y_7}{y_8}}{\lnot(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_4 \end{mlbrace}}
	\newcommand{\XFour}{\hVarX_4 = \hVarX_0}
	\newcommand{\XOne}{\hVarX_1 = \hfls}	
	\newcommand{\XZero}{\hVarX_0 = \begin{mlbrace} \hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5=i}\hVarX_5 \hand\hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5\neq i}\hVarX_5 \\\hand \hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5=i}\hVarX_8 \hand \hgnec{\recv{y_5}{y_6}}{y_6\neq5\land y_5=i}\hVarX_8 \end{mlbrace}}
	
	
	$\gencond{\syseq{\eq^{\alpha}}{\hVarX_{13}}{\sysrecsetE}} \;\; = \;\; \syseq{\gencondEq{\eq^{\alpha}}{\Set{13}}}{\hVarX_{13}}{\sysrecsetE} \quad$   where
	
	$\\\gencondEq{\eq^{\alpha}}{\Set{13}}=\Set{\XThirteen}\;\cup\;\gencondEq{\eq^{\alpha}_1}{Q_1}\\$	
	where $\eq^{\alpha}_1=\eq^{\alpha}\setminus\Set{\hVarX_{13}=F_{13}}$ and $Q_1=\bigunion{i\in\set{13}\hspace{-5mm}}\after{i}\,=\,\Set{11,2}$\\
	
	$\\\begin{array}{rl}
		\gencondEq{\eq^{\alpha}_1}{\Set{11,2}}=&\Set{\XEleven}\;\cup\\&\Set{\XTwo}\cup\gencondEq{\eq^{\alpha}_2}{Q_2}
	\end{array}$\\	
	where $\eq^{\alpha}_2=\eq^{\alpha}_1\setminus\Set{\hVarX_{11}=F_{11},\hVarX_{2}=F_{2}}$ and $Q_2=\bigunion{i\in\set{11,2}\hspace{-5mm}}\after{i}\,=\,\Set{0,1}$\\
	
	$\\\gencondEq{\eq^{\alpha}_2}{\Set{0,1}}=\Set{\XOne}\cup\Set{\XZero}\cup\gencondEq{\eq^{\alpha}_3}{Q_3}\\$ where $\eq^{\alpha}_3=\eq^{\alpha}_2\setminus\Set{\hVarX_{0}=F_{0},\hVarX_{1}=F_{1}}$ and  $Q_3=\bigunion{i\in\set{0,1}\hspace{-5mm}}\after{i}\,=\,\Set{5,8}$\\
	
	$\\\begin{array}{rl}\gencondEq{\eq^{\alpha}_3}{\Set{5,8}}=&\Set{\XFive}\cup\\&\Set{\XEight}\cup\gencondEq{\eq^{\alpha}_4}{Q_4}\end{array}\\$	
	where $\eq^{\alpha}_4=\eq^{\alpha}_3\setminus\Set{\hVarX_{5}=F_{5},\hVarX_{8}=F_{8}}$ and  $Q_4=\bigunion{i\in\set{5,8}\hspace{-5mm}}\after{i}\,=\,\Set{4,7}$ \\
	
	$\\\gencondEq{\eq^{\alpha}_4}{\Set{4,7}}=\Set{\XFour}\cup\Set{\XSeven}\cup\gencondEq{\eq^{\alpha}_5}{Q_5}\\$	
	where $\eq^{\alpha}_5=\eq^{\alpha}_4\setminus\Set{\hVarX_{4}=F_{4},\hVarX_{7}=F_{7}}=\emptyset$  and  $Q_5=\bigunion{i\in\set{4,7}\hspace{-5mm}}\after{i}\,=\,\emptyset$ \\
	
	$\\\gencondEq{\eqE}{\emptyset}=\eqE$	
	
	\noindent $\\[5mm]\therefore$ The Result is $\gencond{\syseq{\eq^{\alpha}}{X_{13}}{\sysrecsetE}} \; =\; \syseq{\eqCond}{X_{13}}{\sysrecsetE}$	 where 	
	
		$$\eqCond = \begin{mlbrack}
			\\\XFour,\hfill\XSeven,\hfill\XOne,\quad\\[1mm]\XThirteen,\\[4mm]\XEleven,\\[4mm]\XEight,\\[4mm]\XFive,\\[4mm]\XTwo,\\[4mm]\XZero
		\end{mlbrack}$$
\end{derivation} \vspace{5mm}

\begin{derivation}[Step 6 - Convert to a Normalized System of Equations using Construction~\ref{sec-sfsys-to-detsys}]
	\normalfont
	\newcommand{\XThirteen}{\hVarX_{\set{13}} = \begin{mlbrace}
			\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_{\color{red}\set{11,2}} \\ \hand \hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!\neq\!i)}\hVarX_{\set{11}} \hand  \hand \hgnec{\recv{y_1}{y_2}}{(y_2\!\neq\!5\land y_1\!=\!i)}\hVarX_{\set{2}}
	\end{mlbrace}}
	\newcommand{\XEleven}{\hVarX_{\set{11}} =  \begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{0}} \hand \\\hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land \lnot(y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{0}}  \end{mlbrace}}
	
	\newcommand{\XElevenTwo}{\hVarX_{\color{red}\set{11,2}} =  \begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\color{red}\set{0,1}} \hand \\\hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land \lnot(y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{0}} \hand \\\hgnec{\recv{y_3}{y_4}}{\lnot(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{1}} \end{mlbrace}}
	
	\newcommand{\XTwo}{\hVarX_{\set{2}} =  \begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{1}}\hand\\ \hgnec{\recv{y_3}{y_4}}{\lnot(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\hVarX_{\set{1}} \end{mlbrace}}	
	\newcommand{\XEight}{\hVarX_{\set{8}} =   \begin{mlbrace} \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_{\set{7}} \hand \\\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land\lnot(y_8>3\land y_7=j)}\hVarX_{\set{7}}\end{mlbrace}}	
	\newcommand{\XSeven}{\hVarX_{\set{7}} = \hfls}
	\newcommand{\XFive}{\hVarX_{\set{5}} = \begin{mlbrace}	\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_{\set{4}} \\\hand \hgnec{\recv{y_7}{y_8}}{\lnot(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_{\set{4}} \end{mlbrace}}
	\newcommand{\XFour}{\hVarX_{\set{4}} = \hVarX_{\set{0}}}
	\newcommand{\XOne}{\hVarX_{\set{1}} = \hfls}	
	\newcommand{\XZeroOne}{\hVarX_{\color{red}\set{0,1}} = \hfls}	
	\newcommand{\XFourSeven}{\hVarX_{\color{red}\set{4,7}} = \hfls}	
	\newcommand{\XZero}{\hVarX_{\set{0}} = \begin{mlbrace} \hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5=i}\hVarX_{\color{red}\set{5,8}} \hand\hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5\neq i}\hVarX_{\set{5}} \\\hand \hgnec{\recv{y_5}{y_6}}{y_6\neq5\land y_5=i}\hVarX_{\set{8}} \end{mlbrace}}
	
	\newcommand{\XFiveEight}{\hVarX_{\color{red}\set{5,8}} = \begin{mlbrace}	\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_{\color{red}\set{4,7}} \\\hand \hgnec{\recv{y_7}{y_8}}{\lnot(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\hVarX_{\set{4}} \\\hand \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land\lnot(y_8>3\land y_7=j)}\hVarX_{\set{7}} \end{mlbrace}}
	
	Since all of our open-guarded patterns are now \emph{distinct}, we are sure that for all necessities guarding the branches of a conjunction, the only case when a system action can satisfy more than one necessity is whenever these necessities are \emph{syntactically equal}. This allows us to encode our open guarded necessities into closed patterns, \eg $\hgnec{\recv{x}{y}}{x=i\land y>5}$ can be encoded as $\hnec{\acta^{(\recv{x}{y},x=i\land y>5)}}$. This encoding allows us to then use the existing determinization algorithm introduce in \cite{Aceto2016Determinization}. In our examples we however omit showing this encoding technique and perform the algorithm directly on the distinct guarded necessities.	
	
	$\\$\noindent The Result is $\gendet{\syseq{\eqCond}{X_{\set{13}}}{\sysrecsetE}} \; =\; \syseq{\eqDet}{X_{\set{13}}}{\sysrecsetE}$	 where 	
	
	$$\eqDet = \begin{mlbrack}
	\\\XFour,\hfill\XSeven,\hfill\XFourSeven,\hfill\XOne,\hfill\XZeroOne,\quad\\[1mm]\XThirteen,\\[4mm]\XEleven,\\[4mm]\XTwo,\\[4mm]\XElevenTwo,\\[4mm]\XEight,\\[4mm]\XFive,\\[4mm]\XFiveEight,\\[4mm]\XZero
	\end{mlbrack}$$
\end{derivation}

\noindent Notice how syntactically equal necessities were \emph{merged together} using this reconstruction. For instance, in $\hVarX_{13}$, branches $\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_{11}$ and $\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_{2}$ were merged together into $\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\hVarX_{\color{red}\set{11,2}}$ since their pattern-guard combination is \emph{syntactically equal} to each other, yet different from that of the remaining ones, \ie $\hgnec{\recv{y_1}{y_2}}{(y_2\!\neq\!5\land y_1\!=\!i)}\hVarX_{2}$ and $\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!\neq\!i)}\hVarX_{11}$. 
\vspace{5mm}

\begin{derivation}[Step 7 - Convert to a \shmlwf formula, using Construction \ref{sec-detsys-to-shml}]
\normalfont
\newcommand{\XThirteen}{\begin{mlbrace}
		\hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!=\!i)}\\\quad\XElevenTwo \hand \\[20mm] \hgnec{\recv{y_1}{y_2}}{(y_2\!=\!5\land y_1\!\neq\!i)}\\\quad\XEleven \hand\\[25mm] \hgnec{\recv{y_1}{y_2}}{(y_2\!\neq\!5\land y_1\!=\!i)}\\\quad\XTwo
\end{mlbrace}}
\newcommand{\XEleven}{\begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\\\quad\hmax{\hVarX_{\set{0}}}{\XZero} \hand \\\hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land \lnot(y_3\!\notin\!\Set{i,j} \land y_4=5)}\\\quad\hmax{\hVarX_{\set{0}}}{\XZero}  \end{mlbrace}}

\newcommand{\XElevenTwo}{\begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\XZeroOne \hand \\\hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land \lnot(y_3\!\notin\!\Set{i,j} \land y_4=5)}\\\quad\hmax{\hVarX_{\set{0}}}{\XZero} \hand \\\hgnec{\recv{y_3}{y_4}}{\lnot(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\XOne \end{mlbrace}}

\newcommand{\XTwo}{\begin{mlbrace} \hgnec{\recv{y_3}{y_4}}{(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\XOne\hand\\ \hgnec{\recv{y_3}{y_4}}{\lnot(y_4>3\land y_3=j)\land (y_3\!\notin\!\Set{i,j} \land y_4=5)}\XOne \end{mlbrace}}	

\newcommand{\XEight}{\begin{mlbrace} \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\XSeven \hand \\\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land\lnot(y_8>3\land y_7=j)}\XSeven\end{mlbrace}}	
\newcommand{\XSeven}{\hfls}

\newcommand{\XFive}{\begin{mlbrace}	\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\XFour \hand\\ \hgnec{\recv{y_7}{y_8}}{\lnot(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\XFour \end{mlbrace}}

\newcommand{\XFour}{\hVarX_{\set{0}}}
\newcommand{\XOne}{\hfls}	
\newcommand{\XZeroOne}{\hfls}	
\newcommand{\XFourSeven}{\hfls}	

\newcommand{\XZero}{\begin{mlbrace} \hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5=i}\XFiveEight \hand\\\hgnec{\recv{y_5}{y_6}}{y_6=5\land y_5\neq i}\XFive \hand\\ \hgnec{\recv{y_5}{y_6}}{y_6\neq5\land y_5=i}\XEight \end{mlbrace}}

\newcommand{\XFiveEight}{\begin{mlbrace}\hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\XFourSeven \hand\\ \hgnec{\recv{y_7}{y_8}}{\lnot(y_7\!\notin\!\Set{i,j}\land y_8=5)\land(y_8>3\land y_7=j)}\XFour \hand\\ \hgnec{\recv{y_7}{y_8}}{(y_7\!\notin\!\Set{i,j}\land y_8=5)\land\lnot(y_8>3\land y_7=j)}\XSeven \end{mlbrace}}

\noindent The final construction consists in substituting the recursion variables with maximal fixpoints. Hence, the Result is $\genwf{\syseq{\eqDet}{X_{\set{13}}}{\sysrecsetE}} \; =\;\hV^{\textsf{wf}}$ where 
\begin{align*}
	&\hV^{\textsf{wf}}=\\&\XThirteen
\end{align*}
\end{derivation}
